Automated Code Optimization with E-Graphs

This thesis proposes an advanced, generic and high-level code rewriting and analysis system in the Julia programming language, providing applied equality saturation in the presence of multiple dispatch and metaprogramming. We show how our system can practically solve some challenging problems: Can programmers implement their own high-level compiler optimizations for their domain-specific scientific programs, without the requirement of them being compiler experts at all? Can these optimizers be implemented by users in the same language and inside the same programs they want to optimize, solving the two-language problem? Can these compiler optimizers be written in a high-level fashion, as equations, without the need to worry about the rewriting ordering? Thus, can symbolic mathematics do high-level compiler optimizations or vice-versa?

==> chapters/unused/pyratesvsmtk.tex <==
\FloatBarrier

\paragraph{Pyrates vs ModelingToolkit}
Another example of the \textit{two-language} problem can be shown in the context of neurodynamical systems modeling. 
\textit{Pyrates} \cite{gast2019pyrates} is an open-source, graph-based Python simulator and parameter analysis toolbox for dynamical systems, designed for the context of neurodynamical models. It uses a Numpy backend for fast simulations of small-medium  networks and a Tensorflow backend for efficient parallelization on GPUs/CPUs, and relies on Fortran for parameter continuations.
Pyrates allows users to define the dynamical systems models with the markup language YAML. This is an evident manifestation of a many-language problem, introducing unelegant and unneeded complexity in the Pyrates system such as additional parsers for the equation definition sub-language.

\todo{Introduce modelingtoolkit}


In \autoref{sec:conductor} we will further investigate the relationship between Julia and Python in the context of neuronal simulation through dynamical system modeling. Precisely, we will investigate the impact of the main contribution of this thesis -- automated symbolic code optimization -- on the performance of such neurodynamical model simulations by comparing how models written in Pyrates perform against optimized and unoptimized models in Conductor.jl, a Julia-based neuronal network simulator engine relying on ModelingToolkit.jl. 


\begin{figure}[h]
    \centering
        \caption{The two-language problem in a dynamical systems modeling context}
    \begin{jllisting}[style=jlcodestyle]
RPO_e:
    base: OperatorTemplate
    equations: ['d/dt * V = V_t',
                'd/dt * V_t = H/tau * m_in - 2 * V_t/tau - V/tau^2']
    variables:
        V:
            default: output
        I:
            default: variable
        m_in:
            default: input
        tau:
            default: 0.01
        H:
            default: 0.00325
    \end{jllisting}
    \subcaption{This piece of Code represents the YAML definition of a rate-to-potential operator in a Jansen-Rit model, a neural population model of a local cortical circuit. The code for solving an instance of the system as a problem is not provided.
    Code from the Pyrates documentation:
    \url{https://pyrates.readthedocs.io/en/latest/auto_interfaces/yaml_definitions.html}}
    \label{fig:yamlrpo}
     \begin{jllisting}[language=julia, style=jlcodestyle]
using ModelingToolkit
using DifferentialEquations: solve
using Plots: plot
@variables t I(t) V(t)
@parameters τ H input
D = Differential(t)
equations = [ 
        D(V) ~ I,
        D(I) ~ H/τ * input - 2I/τ - V/τ^2
]
@named rpo = ODESystem(equations)
prob = ODEProblem(structural_simplify(rpo), [V => 0, I => 0], (0.0, 1.0),
    [τ => 0.12, H => 0.00425, input=>0.5])
sol = solve(prob)
plot(sol, vars=[V, I])
\end{jllisting}
    \subcaption{
    In the same page space, we manage to build the ODE System of the RPO, define an instance of the problem, find the solution and plot it, all without leaving a pure Julia environment.}
    \label{fig:yamlrpo}
\end{figure}

\todo{finish}



